No Calm in The Storm: Investigating QAnon Website Relationships

QAnon is a far-right conspiracy theory whose followers largely organize online. In this work, we use web crawls seeded from two of the largest QAnon hotbeds on the Internet, Voat and 8kun, to build a QAnon-centered domain-based hyperlink graph. We use this graph to identify, understand, and learn about the set of websites that spread QAnon content online. Specifically, we curate the largest list of QAnon centered websites to date, from which we document the types of QAnon sites, their hosting providers, as well as their popularity. We further analyze QAnon websites' connection to mainstream news and misinformation online, highlighting the outsized role misinformation websites play in spreading the conspiracy. Finally, we leverage the observed relationship between QAnon and misinformation sites to build a highly accurate random forest classifier that distinguishes between misinformation and authentic news sites. Our results demonstrate new and effective ways to study the growing presence of conspiracy theories and misinformation on the Internet.

==> dead.tex <==

%\begin{tabular}{|l|c|c|}
%\hline
%\rowcolor{Gray}
%\textbf{Domain/Account} & \textbf{Popularity (Num Followers, Alexa Num)} &  %\textbf{Number of Unique QAnon Links}  \\
% \hline
% \textbf{Bitchute.com}& \multicolumn{1}{r|}{1031}& \multicolumn{1}{r|}{808} \\ \hline
%  \textbf{Endchan.net}& \multicolumn{1}{r|}{NA}& \multicolumn{1}{r|}{636} \\ \hline
%   \textbf{BenjaminFulFord.net}& \multicolumn{1}{r|}{186280} &  %\multicolumn{1}{r|}{242}\\ \hline
% 
%   \textbf{citizensamericaparty.org}& \multicolumn{1}{r|}{NA} & %\multicolumn{1}{r|}{168} \\ \hline 
%       \textbf{realjewnews.com}&\multicolumn{1}{r|}{NA} & \multicolumn{1}{r|}{132}\\ %\hline  % the lion of juday daily 
%  \textbf{vultureofcritique.wordpress.com}& \multicolumn{1}{r|}{NA} %&\multicolumn{1}{r|}{109}\\ \hline  % the lion of juday daily 
%    \textbf{cathyfox.wordpress.com}&\multicolumn{1}{r|}{NA} & \multicolumn{1}{r|}{93}\\ %\hline  % the lion of juday daily 
%  \textbf{Twitter User 1 }& \multicolumn{1}{r|}{566K}&\multicolumn{1}{r|}{282}  \\ %\hline % x22 report
%  \textbf{Twitter User 2}& \multicolumn{1}{r|}{12.8K}& \multicolumn{1}{r|}{264} \\ %\hline %@rqueenic jim
%    \textbf{Twitter User 3}& \multicolumn{1}{r|}{502}& \multicolumn{1}{r|}{183}\\ %\hline %wins of the day 
%    \textbf{Twitter User 4}& \multicolumn{1}{r|}{29.5K} &\multicolumn{1}{r|}{142}\\ %\hline % % american patriot 
%    \textbf{Twitter User 5}& \multicolumn{1}{r|}{8,120} &\multicolumn{1}{r|}{138}\\ %\hline  % the lion of juday daily 
%    \textbf{Twitter User 6}& \multicolumn{1}{r|}{428K} &\multicolumn{1}{r|}{26}\\ %\hline  % tpatriot1776����
%\end{tabular}
%\caption{\label{tab:graph-information} We note the domains with the most unique links %to QAnon domains. We consider QAnont domains to be those that are dedicated to QAnon %content. Examples include qanon.pub, qagg.news, etc. }
%\end{table}


%\subsubsection{bitchute.com:} BitChute is a video housing service renown for hosting far-right %materials and conspiracy theorists. The Southern Povery Law Center has labeled the stie as %hosting ``hate-fueled material" and Twitter started blocking posts linking to the stie in August %2020. Given that the majority of YouTube videos linked from 8kun.top and voat.co have now been %blocked, BitChute appears to fulfilling its roles allowing conspiracy to spread on its platform. %As the largetest domain besides twitter directing users to QAnon content, it plays a pivotal %role.
%
%\subsubsection{endchan.net:} EndChan is an imageboard that promotes the message 'this is the end' %or the end of the universe. Like 8kun.top, endchan.net has become home to QAnon content with %board dedicated to QAnon research and discussion.
%
%\subsubsection{realjewnews.com:} An important aspect of QAnon according the Anti Defamation %League is Anti-Semitism. The fact that this site in particular is one of the largest in terms of %unique links concurs with the ADL's finding. 
%
%\subsubsection{wordpress sites:} Both cathyfox.wordpress.com and vultureofcritique.wordpress.com %are user web-pages that circulate misinformation. cathyfox.wordpress.com is geared towards %uncovering information about child traficking while vultureofcritique.wordpress.com is geared %toward general crime.
%
%\subsubsection{benjaminfulford.net:} Benjamin Fulford is ostensibly a Canadian-Japanese %journalist who appears to peddle in conspiracy theories. 
%
%\subsubsection{Alternative News Sites:} There are a list of alternative news sites including %\texttt{thegatewaypundit.com}, \texttt{zerohedge.com}, \texttt{americanthinker.com}, %\texttt{pjmdia.com}, and \texttt{breitbart.com} that play a role in redirecting users to QAnon %content. 
%
%\subsubsection{Mainstream News Sites:} There are a list of relatively mainstream sites that also %have links back to QAnon related materials. These sites most have linked back to %\texttt{8kun.top} in news stories. The list include notable sites like \texttt{reuters.com}, and %\texttt{usatoday.com}. Given that \texttt{google.com} has taken steps to remove these sites from %their search results and extremist content on these sites, we recommend that these sites also %take steps to remove them from their domains. 
%
%Except for BitChute, many of the websites directed users to QAnon content sites are relatively %unknown; however, several popular websites without user generated content still have direct links %back to Q sites. \texttt{thegatewaypundit.com} (Alexa 377), \texttt{heavy.com} (Alexa 309), %\texttt{breitbart.com} (Alexa 316), \texttt{zerohedge.com} (Alexa 377), and  \texttt{google.com}. %For a comprehensive list of websites that direct users through links back to QAnon content, %please email us. 




\begin{center}
\begin{table}[ht]
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{|l|r|l|r}
\hline
\rowcolor{Gray}
\textbf{Hashtag}  &  \textbf{Number of Hashtags/Percentage} & \textbf{Website Domain}  &  \textbf{Number of Links/Percentage}  \\
 \hline
 \textbf{qanon}& \multicolumn{1}{r|}{2787/ 2.92\%} & \textbf{youtube.com}& \multicolumn{1}{r|}{14830/ 21.00\%} \\ \hline
\textbf{wwg1wga}& \multicolumn{1}{r|}{1620/ 1.70\%} & \textbf{thegatewaypundit.com}& \multicolumn{1}{r|}{1789/ 2.53\%}\\ \hline
\textbf{maga}& \multicolumn{1}{r|}{1603/ 1.68\%}& \textbf{breitbart.com}& \multicolumn{1}{r|}{1726/ 2.44\%} \\ \hline
\textbf{fightback}& \multicolumn{1}{r|}{1277/ 1.34\%}& \textbf{rumble.com}& \multicolumn{1}{r|}{1523/ 2.16\%} \\ \hline
\textbf{stopthesteal}& \multicolumn{1}{r|}{1017/ 1.07\%} & \textbf{pscp.tv}& \multicolumn{1}{r|}{1512/ 2.14\%}\\ \hline
\textbf{trump2020}& \multicolumn{1}{r|}{936/ 0.98\%}& \textbf{theepochtimes.com}& \multicolumn{1}{r|}{1451/2.06\%} \\ \hline
\textbf{fakenews}& \multicolumn{1}{r|}{874/ 0.92\%}& \textbf{nypost.com}& \multicolumn{1}{r|}{1189/ 1.68\%} \\ \hline
\textbf{covid19}& \multicolumn{1}{r|}{840/ 0.88\%} & \textbf{washingtonexaminer.com}& \multicolumn{1}{r|}{1049/ 1.49\%}\\ \hline
\textbf{wethepeople}& \multicolumn{1}{r|}{828/ 0.87\%}& \textbf{bitchute.com}& \multicolumn{1}{r|}{1046/ 1.48\%} \\ \hline
\textbf{foxnews}& \multicolumn{1}{r|}{715/ 0.75\%}& \textbf{foxnews.com}& \multicolumn{1}{r|}{1043/ 1.48\%} \\ \hline
\textbf{georgia}& \multicolumn{1}{r|}{668/ 0.70\%} & \textbf{zerohedge.com}& \multicolumn{1}{r|}{796/ 1.13\%}\\ \hline
\textbf{fightfortrump}& \multicolumn{1}{r|}{608/ 0.64\%}& \textbf{thefederalist.com}& \multicolumn{1}{r|}{646/ 0.91\%} \\ \hline
\textbf{breaking}& \multicolumn{1}{r|}{571/ 0.60\%} & \textbf{justthenews.com}& \multicolumn{1}{r|}{634/ 0.90\%}\\ \hline
\textbf{trump}& \multicolumn{1}{r|}{564/ 0.59\%} & \textbf{dailymail.co.uk}& \multicolumn{1}{r|}{593/ 0.84\%}\\ \hline
\textbf{coronavirus}& \multicolumn{1}{r|}{560/ 0.59\%} & \textbf{babylonbee.com}& \multicolumn{1}{r|}{483/ 0.68\%}\\ \hline
\textbf{obamagate}& \multicolumn{1}{r|}{542/ 0.57\%} & \textbf{facebook.com}& \multicolumn{1}{r|}{474/ 0.67\%}\\ \hline
\textbf{stopthesteai}& \multicolumn{1}{r|}{494/ 0.52\%} & \textbf{newsmax.com}& \multicolumn{1}{r|}{444/ 0.63\%}\\ \hline
\textbf{china}& \multicolumn{1}{r|}{481/ 0.50\%} & \textbf{fllwrs.com}& \multicolumn{1}{r|}{439/ 0.62\%}\\ \hline
\textbf{thegreatawakening}& \multicolumn{1}{r|}{448/ 0.47\%}& \textbf{x22report.com}& \multicolumn{1}{r|}{423/ 0.60\%} \\ \hline
\textbf{digitalsoldiers}& \multicolumn{1}{r|}{414/ 0.43\%} & \textbf{tora3.com
}& \multicolumn{1}{r|}{387/ 0.55\%}\\ \hline
\end{tabular}}
\caption{\label{tab:graph-information} (Left)The top hashtags of the 95263 unique hashtags for accounts within the QAnon Twitter network. As seen while many are directly related to the QAnon movmement, others are concerned with current events (the 2021 Georgia Senate Runoff) and conservative election preferences( \texttt{i.e.} trump2020). (Right) The top domains linked by QAnon related accounts after excluding other twitter accounts and tweets linked. As seen in, the list include many more mainstream sources.  }
\end{table}
\end{center}


An alternative version of Facebook was found in \textit{spreely.com} (Alexa 155019). An alternative and now infamous twitter clone was found in \textit{parler.com} (Alexa 903). Finally an app to read twitter conversations was found in \textit{threadreaderapp.com}. We note that in particular that \texttt{poal.co} (Alexa 201961),has two different subreddits dedicated to QAnon. We lastly list a IRC channel apparently dedicated to \textit{voat.co} in \textit{goat.chat}. We lastly note a do









%In this section, we use our hyperlink graph to broadly understand the sites that host QAnon content and how users reach them. We analyze the sites most posted on 8kun and Voat, we identify a set of 126~QAnon focused websites that act as secondary hubs of QAnon content, we discuss how mainstream websites like Twitter and Youtube play a significant role in the ecosystem, and we show how the hyperlink graph can be used identify newly established QAnon domains and other misinformation websites.

%\begin{table*}
%\centering
%\small
%\begin{tabular}{lrrrrrr}
%\toprule
%{Domain} & {Hub} & {Authority} & {Eigen. Central}  & {Betw. Central} & {In-Deg.} & {Out-Deg.} \\
% \midrule
% {voat.co}   &   0.306085    &   0.023722    &   0.031302    &   0.089498    &   69  &    7,207 \\ 
% {bitchute.com}   &   0.288944    &   0.038224    &   0.071622    &  0.026752    &   246  &    4,836 \\ 
% {twitter.com}   &   0.286305    &   0.124899    &   1.0    &   0.36832    &   4,621  &    4,659  \\ 
% {8kun.top}   &   0.239276    &   0.019919    &   0.027432    &  0.129418    &   67  &    6,802 \\ 
% {stillnessinthestorm.com}   &   0.217002    &   0.016277    &   0.019585    &   0.003426    &   26  &    2,693 \\ 
% {wordpress.com}   &   0.191538    &   0.053875    &   0.160252    &   0.027245    &   633  &    2,296 \\ 
% {wikipedia.org}   &   0.189265    &   0.059812    &   0.193066    &   0.020393    &   731  &    2,625 \\  
% {fellowshipoftheminds.com}   &   0.156442    &   0.018782    &   0.021317    &   0.001353    &   35  &    1,674 \\ 
% {truth11.com}   &   0.286305    &   0.153406    &   0.016401    &   0.001466    &   17  &    1,632  \\ 
% {conservapedia.com}   &   0.286305    &   0.019401    &   0.025599    &   0.001618    &   35  &    1,515 \\ 
% \bottomrule
%\end{tabular}
%\caption{\label{tab:8kun-voat-hubs} Major Hubs within the Voat-8kun network graph with their centrality characteristics.  \todo{How are these defined as major? Is it somehow a top 10? What am I supposed to take away from these numbers? Can you label which of the four types each is? I suspect that a top ten within each category would be more meaningful. I don't think that these numberic values are helpful to the reader. If anything they belong in the appendix of an extended version of the paper.}}
%
%\end{table*}
%\begin{enumerate}
%    \item The hub of contents and information that surround the QAnon boards of \texttt{8kun.top} and \texttt{voat.co} and identifying the different types of domains that participate in this network. We find that a large collection of alternative news distes, video sharing domains, and personal blogs play a large role in the QAnon universe. Similarly, although ostensibly known, we find that Twitter plays an outsized role within the network surrounding \texttt{8kun.top} and \texttt{voat.co}.
%    \item The existence and role of a collection of 126 QAnon focused sites besides the ``official" homes of \texttt{8kun.top} and \texttt{voat.co}. The popularity of these domains mirror several interventions several social media companies and give an of the popularity of the QAnon movement.  We further document the large role that several  media companies (primarily \texttt{twitter.com}, \texttt{youtube.com}, and \texttt{bitchute.com}) have in provided content for the QAnon movement. 
%    \item The use of our larger hyperlink graph in identifying additional QAnon domains and to identify new misinformation sites. We find that exceedingly few domains have links back to QAnon content sites. Given the toxicity of the conspiracy theory, we find high utility in utilizing our extended hyperlink graph in identifying additional QAnon domains and misinformation sites. 
%\end{enumerate}

%\subsection{Sites Linked from 8kun and Voat}


%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{figures/voat8kuninout.png}
%\caption{\todo{there needs to be a description that this is what voat/8kun links to.} 203 Largest content hubs in \texttt{voat.co} and \texttt{8kun.top} content network. Full graph continas 12,325 nodes and 144,826 different connections. Color in graph determined by by Louvain clustering algorithm. 
%\todo{what's the point/takeaway from this graph? Why should I care about the colors? Can you label the clusters on the graph? It looks like you know what they are in the text.} \todo{What \% of links go to each of the four categories?} \todo{pdfcrop}
%}
%\label{fig:voat-8kun-sub}
%\end{figure}

%\paragraph{Social Media (Purple).} 
%\todo{Quantify the roles that these sites play!!!! There isn't very much any content here that we couldn't have simply naively guessed. What have we learned \textbf{quantitatively} about how social media sites play a role? What \% of links are to social media sites? Is this in a table somewhere? What is the type of content being linked to? What subreddits are linked to? Does Reddit decrease with time post ban? It'd be interesting to see what all of these look like temporally? Are they linked to individual posts? Are they posted in a positive or negative way?}

%\todo{Why are they links to twitter? Are there major accounts repeatedly being linked? Subreddits? Do those accounts link back to this content? Why have we classified Google and Wikipedia as social media sites? \emph{Why} are they linking to Twitter? What does that mean about Twitter?}

%\todo{What are we supposed to take away from this paragraph? What does \emph{large} role mean? Can you quantify that? Are the accounts linked different from the ones mentioned in prior studies of Twitter? Why does being linked to make you a ``hub'' of content? Is it the content itself or simply discussion of it? How much twitter content is republican stuff, or is it more q-anon-y? Same for wikipedia. Why are people linking to that? Can you provide a sentence or two of intuition?}

%Mainstream social media sites play a significant role in the QAnon ecosystem, most notably Twitter and Reddit, which are the first and third largest hubs beyond 8kun and Voat~\todo{does that simply mean they're most linked? If so, just say that.} and account for \TK\% of links posted to the two aggregators. Given that Reddit struck down many of its QAnon focused subreddits in the Summer of 2018, its much smaller role here is understandable.\todo{NO NO NO! Don't just say that. \textbf{SHOW ME THAT}. You have the data from after Reddit banned the Subreddits. Show that when that happened, the number of links to Reddit content plummeted. Show that it was successful.} \todo{add graph of all social media site links over time. I expect we'll start to see Parler increase etc.} There are few links to Faccebook and Parler, which rank \todo{where? quantify.} \todo{do we have any sense why?} \todo{still want to know what those all look like temporally.} More than 3,000~Twitter accounts are linked~\todo{add of cdf of twitter accounts, subreddits, wordpress sites, etc. that have coverage of all links from the aggregators and probably a table of the top ten of each.}.


%The prevalence of \texttt{twitter.com} is evinced by the nearly 3000 different Twitter accounts referenced within our scrape of \texttt{8kun.top} and \texttt{voat.co}. Given that President Donald Trump plays a large role in the QAnon conspiracy theory and twitter remains one of his most prominent vehicles for communication, the role that twitter would play was obvious.\todo{It's really not. Never say something is obvious in a research paper. Either show us with data or do not make the claim. Are all of these linking to Donald Trump tweets?}

%We see a much smaller role for \texttt{reddit.com}. 

%Given that they required log-ins to scrape or outright disallowed scraping in their terms of service, tere lack of contribution to this initial graph does not absolve them. As we will see later, they play a large role in the larger QAnon network. 

%\paragraph{Alternative Media and News Sites (Blue)} More than \TK\% of links on 8kun and Voat are to alternative media sites, as defined by Snopes, FakeNewsChecker, and Melissa Zimdars' list~\cite{TK}. \todo{quantify number of sites. a CDF might help here.} \todo{move these to a table, add quantitative data, and ref: \textit{washingtonexaminer.com}, \textit{dailywire.com}, \textit{dailycaller.com}, \textit{thegatewaypundit.com}, \textit{truepundit.com}, \textit{breitbart.com}, \textit{wnd.com}, \textit{rt.com}, \textit{whatdoesitmean.com}, \textit{freebeacon.com}, \textit{newswithviews.com}, and \textit{zerohedge.com}.} \todo{This list only seems to be a very small set of the Blue cluster. There are also a bunch of seemingly \emph{very} large hubs in that cluster that are never discussed: conservapedia, thereadreaderapp.com, radiopatriot.net, noqreport.com, etc. You need to discuss what these are. Right now there's little sense of why this is such a large cluster or that there's this huge long-tail of sites, which seems like it's a big deal.} \todo{which of these are things that haven't been described in prior literature?}

%fakenewschecker.com labels these site as conspiratorial with the majority (all except rt.com) exhibiting a right leaning bias.\todo{Is this the right link? That site doesn't seem to exist / is just adware. Also, is this \emph{all} of them in the cluster, or just the ones in your list above? What \% of all of them fail the fake news checker test?} We also find \todo{quantify} links to mainstream media sources including the NY Times (\TK\%), Guardian (\TK\%), and Washington Post (\TK\%). While not necessarily spreading QAnon disinformation, these domains link back to 8kun, are linked to by other domains \todo{what other domains?}, and thus play a role in the QAnon network. For example, \todo{provide an example or two about how these news sources are linking back.} Other notably examples include Forbes and Business Insider.\todo{why are these notable and not in the prior set? Do they not link back?} \todo{have we verified how many of these are actually news sites? The difference between this cluster and the orange one seems a bit tenuous.}

%\paragraph{Large Repositories of Extreme Content (Green)} \todo{again quantify.} The last cluster of domains primarily consists of large stores of extreme content as exemplified by 8kun.\todo{How does this work when 8kun is also where we started? Is it that Voat has lots of links to it? Does 8kun have self-referential links? I think you need to explain since it's weird to talk about your starting point being big} Like 8kun, these repositories store different types of extreme content \todo{like what? video? images?} and are not restricted to QAnon information. \todo{provide a couple of examples. there aren't very many so it seems like you could simply describe these.} This further includes one the largest homes of extreme material \texttt{bitchute.com}, which the Southern Poverty Law Center noted in 2019 as being filled  ``hate-fueled material'', and the Anti-Defamation League wrote in 2020 has become hotbed for ``violent, conspiratorial and hate-filled video propaganda''~\cite{TK}. \todo{what are the other things that aren't content stores? there aren't many other things in the cluster, can you just tell us?}

%\paragraph{Individually-Run Websites (Orange)} \todo{quanitify!!} We thirdly note a large collection of small-organization run websites that all play a dominant role in the ecosystem, including \TK Wordpress and \TK Blogger sites. \todo{move this into a table and quantify:} We again identified the most prominent set of domains in this cluster using our list of ``fake news". These include \textit{blacklistednews.com} (inciteful), \textit{henrymakow.com} (conspiratorial), \textit{globalresearch.ca} (conspiratorial), \textit{humansarefree.com} (conspiratorial), \textit{lewrockwell.com} (inciteful), \textit{corbettreport.com} (conspiratorial), \textit{rumormillnews.com} (editorial, inciteful), \textit{rense.com} (conspiratorial, editorial, inciteful), \textit{ sott.net} ( conspiratorial, editorial, inciteful), \textit{darkmoon.me} (conspiratorial), \textit{geoengineeringwatch.org} (psuedoscience), \textit{politicalvelcraft.org} (conspiratorial). \todo{do you have alexa rank data to back up that these are small sites? Are they blogs? Something else? Can you describe how they're different from small news sites?} 


%\texttt{centipedenation.com} does ``reporting on great awakening'' according to its %twitter account. The ``great awakening'' is the belief among QAnon believers that %people across the world are ``awakening'' to the conspiracy that a pedophile ring %controls the world.  \texttt{nukepro.net} is alternative news site that alternative %news sites that promotes conspiracy theories, updates about the QAnon conspiracy, and %misinformation about COVID-19. \texttt{vcbestor.blogpost.com} is a blog that promotes %political conspiracy and the QAnon movement. \texttt{9east71.home.blog} is a blog %dedicated to uncovering pedophilia. The wordpress sites are a mixture of QAnon and %far-right conspiracy sites \textit{ thegodofrage.wordpress.com,
%vultureofcritique.wordpress.com, thanatopianinstitute.wordpress.com, %flyingcuttlefish.wordpress.com, cathyfox.wordpress.com, pal29501.wordpress.com, %homelesszombieapocalypse.wordpress.com, qanonpress.wordpress.com, %dcpizzagate.wordpress.com, goodnessandharmony.wordpress.com}.

\begin{table}
    \centering
    \small
    \begin{tabularx}{\columnwidth}{Xrr}
        \toprule
        Domain      &   Alexa Rank      &  $\rightarrow$ QAnon Domains    \\
        \midrule
        twitter.com         &   42              &   53 (42.1\%) \\
        wordpress.com         &   66              &   46 (36.5\%) \\
        github.com         &   113              &   5 (4.0\%)    \\
        bitchute.com         &   1,522             &   68 (54.0\%) \\
        pastebin.com         &   5,679              &   13 (10.3\%) \\
        x22report.com         &  12,573             &   11 (8.7\%) \\
        americanthinker.com        &   12,964             &   5 (4.0\%) \\
        threadreaderapp.com        &   23,836    &   16 (12,7\%) \\
        theconservativetreehouse.com       &   26,092              &   5 (4.0\%)  \\
        unz.com        &   12,964             &   13 (10.3\%) \\
        \bottomrule
    \end{tabularx}
    \caption{\textbf{Popular domains that point to QAnon}---%
        We show the top popular domains that point directly to at least QAnon domains in the cluster (excluding \texttt{voat.co} and \texttt{8kun.top} ). Many popular social media sites and platforms are used by the QAnon movement to host content, highlighting the role such platforms play in continuing its spread.
    }
    \label{table:popular_domains_to_qanon}
\end{table}

\begin{table}
    \centering
    \small
    \begin{tabularx}{0.48\columnwidth}{Xrr}
    \toprule
    Domain    &  Links    &   \% \\
    \midrule
        twitter         &   1,898         &  33.4\% \\
        bitchute        &   829          &   14.6\% \\
        wordpress       &   355         &   6.25\% \\
        benjaminfulford          &   247          &   4.34\% \\
        citizensamericaparty            &   168          &    2.96\% \\
        realjewnews         &   139          &    2.44\% \\ 
        nukepro         &  94          &    1.85\% \\ 
        %wordpress       &   60.2K           &    1.70\% \\
        %blogger         &   55.9K           &    1.60\% \\
        %8kun            &   38.2K           &    1.10\% \\
        %wikileaks      &   36.4K           &    1.05\% \\
    \bottomrule
    \end{tabularx}
    \begin{tabularx}{0.48\columnwidth}{Xrr}
    \toprule
    Domain    &  Links    &   \% \\
    \midrule
        %twitter         &   1.27M         &   36.52\% \\
        %facebook        &   377K          &   10.84\% \\
        %reddit          &   361K          &   10.39\% \\
        %voat            &   335K          &    9.64\% \\
        %youtube         &   105K          &    3.02\% \\ 
        nukepro         &  94          &    1.66\% \\ 
        2012portal.       &   84           &    1.48\% \\
        abeldanger.         &   73          &    1.29\% \\
        themillenniumreport            &   67           &    1.18\% \\
        threadreaderapp      &   60          &    1.05\% \\
        home.blog           & 53             & 0.93\% \\
        other           & 51              & 26.5\% \\
    \bottomrule
    \end{tabularx}
    \caption{\textbf{Top Domains with links to the QAnon cluster}}
    \label{table:qanon_inwards}
\end{table}


This indicates that connections to QAnon domains or connections to domains that QAnon domains have connections with can divulge details about the semantic content of a given websites. Noticing this trend, we thus  determine that we can utilize features from QAnon domains in order to categorize and label other websites in our network graph as either \textbf{disinformation} or \textbf{authentic}.  We thus utilize our DEEPCRAWL network in order to build an automatic classifier of websites as \textbf{disinformation} or \textbf{authentic} news. 
